MS-HuBERT: Mitigating Pre-training and Inference Mismatch in Masked Language Modelling methods for learning Speech Representations

In recent years, self-supervised pre-training methods have gained significant traction in learning high-level information from raw speech. Among these methods, HuBERT has demonstrated SOTA performance in automatic speech recognition (ASR). However, HuBERT's performance lags behind data2vec due to disparities in pre-training strategies. In this paper, we propose (i) a Swap method to address pre-training and inference mismatch observed in HuBERT and (ii) incorporates Multicluster masked prediction loss for more effective utilization of the models capacity. The resulting method is, MS-HuBERT, an end-to-end self-supervised pre-training method for learning robust speech representations. It beats vanilla HuBERT on the ASR Librispeech benchmark on average by a 5% margin when evaluated on different finetuning splits. Additionally, we demonstrate that the learned embeddings obtained during pre-training encode essential information for improving performance of content based tasks such as ASR.

==> sections/literaturesurvey.tex <==



% Recently data2vec emerges as one model for 3 modalities: vision, speech and text. The learned representations for speech when finetuned in low resoruce settings beat the previous state-of-the-art (SOTA) method i.e., HuBERT \cite{hsu2021hubert}. When evaluated as a feature extractor on a series of speech task on the SuPERB benchmark HuBERT Base outperforms data2vec as shown in Figure \ref{fig:hubertvsdata2vecbase} except on the tasks which require content information.
% Two reasons for this could be: data2vec tokens are continuous and stable. Whereas HuBERT tokens are discrete and noisy. Secondly, during pre-training HuBERT has access to the full context to predict the masked tokens. 

% A recent work by \cite{yadav2023analysing} shows improvement on the content based tasks such as PR and ASR. For PR they even beat the data2vec and for ASR they are close but not have beaten the data2vec. One reason for this is that they trained on a lower batch size, half the batch size of the original HuBERT or data2vec, to precise of the original HuBERT and 1/5th of the learning rate. 

% Based on these observations. In this work, we combine the full context and multiple MLM loss layers to improve the content information further. This is the closest one to one comparison to the data2vec and HuBERT. 


% Our proposed model is better able to model the different granularity of information needed for different tasks in the learned embeddings at different layers. Compared to the data2vec which applies a mean of layers to model them at the last layer only. Our method models the different granularity required separately. Also, since our tokens are noisy but using multiple is helpful, which can to some extent alleviate this problem. 




==> sections/relatedworks.tex <==
\noindent \textbf{Multiple cluster centers}: 
Using multiple cluster centers, also called multiple resolutions, has been investigated by \cite{shi2023explorationMRHUBERT, shi2023MRHuBERT, yadav2023analysing}. 
In \cite{shi2023MRHuBERT}, the author introduces down-sampling and up-sampling modules within the transformer encoder after each layer to facilitate learning features at multiple resolutions. On the other hand, \cite{shi2023explorationMRHUBERT} explores parallel and hierarchical variations of HuBERT with findings indicating the superiority of the hierarchical approach. This involves training multiple models, each model adds almost same parameters as the original HuBERT, at various resolutions using CNN as a down-sampling module. Lastly \cite{yadav2023analysing} uses the fact that MPL is applied at multiple layers of for different resolutions. This method does not introduce any additional parameters to the original HuBERT model, except the linear layers used for loss calculation which are discarded after the pre-training. In this work, we adopt this approach and modify it for our use case of multicluster loss.

% while achieving superior performance on the ASR task.

% the approach outlined in \cite{yadav2023analysing} to incorporate cluster centers at multiple resolutions across multiple layers. 

% In this study, we adopt the approach outlined in \cite{yadav2023analysing} to incorporate cluster centers at multiple resolutions across multiple layers. Remarkably, this method does not introduce any additional parameters to the original HuBERT model while achieving superior performance on the ASR task.


\noindent \textbf{Swap}: 
Using two views of the input is a common practice in the field of computer vision  \cite{chen2020simplesimclr, he2020momentummoco, grill2020bootstrapbyol}. Given $e$ layers in a encoder, it is a general practice to add a similarity loss on the output embeddings of the encoder after each layer, as seen in works using U-net type architectures \cite{ronneberger2015unet1,riahi2023singleunetconcatenate,macartney2018improvedunetconcatenate2}. In contrast, we propose a Swap method which switch the output embeddings, at certain indices, after each layer of the encoder between the masked and unmasked view of the input. This is motivated by the simple fact, that the learned model is expected to generate the same output embeddings regardless of the two views. Swap method addresses the challenging case of the pre-training and inference mismatch in HuBERT by using both the masked and unmasked views during pre-training.




% \textbf{HuBERT,  w2v bert and WavLM paper}: 
% HuBERT \cite{hsu2021hubert} made the masked language modelling technique popular to learn high-level speech representations from raw audio. The idea of HuBERT is pretty simple and is divided in two two stages: (i) In stage 1, given MFCC features, from raw audio, learn a K-means clustering model of a given cluster size, 100 was used in the original paper. Map the raw audio, chunks, to one of cluster label also called as pseudo-labelling. Lastly, the x/y pair (raw-audio/pseudo-labels), is similar to the NLP setting, where the output is discrete. Therefore, the authors of HuBERT uses the BERT pre-training as from NLP. One noticeable change is, the masking technique. In BERT, 15 \% of the tokens are masked, but in HuBERT almost 50\% of the tokens are masked. Simple answer is to make the task harder. Long answer is because speech signal is of very high frequency, therefore neighbouring speech samples contain a lot of information. And thus to learn meaningful representations of the masked indices, we need to mask longer continuous segments in speech. Notably, the authors of HuBERT did not use any data-augmentation. That's what exactly the authors of WavLM \cite{chen2022wavlm} paper did i.e., they augmented the input audio with another audio in the batch (or noise) with certain probability. Given an audio sample, (i) choose with a certain probability to augment the sample or not. (ii) randomly sample 50\% of the segment to augment. (iii) randomly choose the SNR between a range and add the two audios. This simple data-augmentation resulted in the performance boost on speaker based tasks. Lastly, w2v-BERT \cite{chung2021w2vbert}combines MLM loss, from HuBERT, and contrastive loss, from Wav2Vec2.0, for joint optimization. Briefly, the architecture has 24 layers, the authors applied contrastive loss at layer 12 and MLM loss at the 24 layer. One distinction from HuBERT is that the token ids for the MLM loss are learnt during the training using the Wav2Vec2.0 quantization. The authors say that this online quantization with MLM leads to mode collapse i.e., all the masked indices are mapped to one id. This results in zero loss and perfect fit. 


% \textbf{Wav2Vec series paper vq-wav2vec, discreret bert}: 

% In this series of work, different authors study the role of quantization in the learning high level representations starting with the Wav2vec (w2v) \cite{schneider2019wav2vec}. w2v builds upon this idea that meaningful representations of audio can be learned using a contrastive loss. That is to say given an audio $(x)$ and 2 function approximators $f1 and f2$. $f1(x)$ can be used as targets for comparing to predictions of $f2$. Which representation of target is better,continuous or quantized , for the task of ASR, is the focus of study in this series of papers. The first work used is w2v, where the authors use continuous targets and show significant gains for the ASR task in low resource settings. Building on this, vq-w2v \cite{vqw2v} is proposed where the authors quantize the $f1(x)$, either using Gumbel softmax or K-mean clustering, and then fed to the $f2$ and also use as the targets. After this the authors train a BERT \cite{devlin2018bert} over the learned vocabulary. This is a 2 step pre-training process. W2v is still better than vq-w2v but vq-w2v combined with BERT gives significant gains over w2v. K-mean clustering performs significantly better with large number of codewords without the BERT. With the combined pre-training gumbel and k-means perform similarly. Discrete/Continuous BERT takes it one step further and compares quantized and continuous input in the BERT pre-training. Their findings suggest quantization is necessary to achieve good ASR performance specially in the case of low resource settings i.e., first learn a discrete vocabulary of the data with
% vq-wav2vec followed by standard BERT training over these discrete units. This performs much better than directly learning from the continuous audio data. Building on all the previous findings is built w2v2.0 \cite{baevski2020wav2vec2.0}. The authors learn a feature $q$ from $f1(x)$ and then use these features as the input to $f2$, in which they mask around 50\% of the indices. Then learn a vocabulary by quantizing the $q$ using Gumbel softmax and apply a contrastive loss similar to w2v but only on the masked indices. The authors use transformer architecture, a powerful function approximator, to model $f2$. Discrete BERT is the closest model to w2v2.0 and they show that jointly optimizing of w2v and BERT beats Discrete BERT by a large margin on low resource settings. The authors also study the quantized inputs to $f2$ and continuous targets. Continuous input is detrimental to the performance of ASR compared to the targets. Continuous inputs, quantized targets gives the best performing model. 


% \textbf{data2vec series paper and CoBERT paper}

% In this series of paper the authors, propose a  teacher student model such that the teacher can see the complete audio without any artifact as in masking. A student model is fed the masked input similar to the w2v2.0 \cite{baevski2020wav2vec2.0}. The targets for the masked indices are formed by averaging multiple layers of teacher model and then L1 loss is applied between the student predictions and the targets.  This is data2vec pipeline \cite{baevski2022data2vec}. In CoBERT \cite{meng2022cobert}, the authors replace the waveform encoder of data2vec, with a k means word embedding layer in the teacher model, Everything else is same. This change forces more language information in the final learnt model because of its discrete teacher. They show that this setup is good for speech translation and ASR giving improvements over data2vec.


% \textbf{Whisper}: It is a semi supervised method at scale. NO unsupervised or self supervised learning. 

% \textbf{paSE}: common encoder to solve various task parallel, similarly to multi task learning but no need of annotated data, the tasks are defined from using only the unlabelled dataset. 

% \textbf{paSE+:} built on pase but with distorted input, similarly to the TERA idea. 

% \textbf{DeCoAR 2.0:} using quatization and then doing reconstruciton of the masked input using L1 loss. 
% % Modified CPC

% \textbf{TERA:} A Masked prediction method that alters the input and then do the reconstruction. very similar to mockinjay. (Read in detail, also read papers in detail from superbbenchamark such that what techniques are giving better results for specker based tasks. )

% \textbf{Mockinjay}: A Masked prediction method that Uses BERT as it is on continuous speech features. Different than wav2vec as their is no contrastive loss. 

% % FAST-VGS+

% % autoregresive prediction mehtod or contrastive method (wav2vec). 
